Semi-Federated Scheduling of Parallel Real-Time Tasks on Multiprocessors

Federated scheduling is a promising approach to schedule parallel real-time tasks on multi-cores, where each heavy task exclusively executes on a number of dedicated processors, while light tasks are treated as sequential sporadic tasks and share the remaining processors. However, federated scheduling suffers resource waste since a heavy task with processing capacity requirement $x + \epsilon$ (where $x$ is an integer and $0 < \epsilon < 1$) needs $x + 1$ dedicated processors. In the extreme case, almost half of the processing capacity is wasted. In this paper we propose the semi-federate scheduling approach, which only grants $x$ dedicated processors to a heavy task with processing capacity requirement $x + \epsilon$, and schedules the remaining $\epsilon$ part together with light tasks on shared processors. Experiments with randomly generated task sets show the semi-federated scheduling approach significantly outperforms not only federated scheduling, but also all existing approaches for scheduling parallel real-time tasks on multi-cores.

==> define_back.tex <==
\newcommand{\todo}[1]{\textcolor[rgb]{1.00,0.00,0.00}{GUAN: #1}}

\newcommand{\forget}[1]{}

\newtheorem{observation}{Observation}
\newtheorem{lemma}{Lemma}
\newtheorem{define}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{strategy}{Strategy}

\newcommand{\dbf}{\textsf{\upshape{dbf}}}
\newcommand{\df}{\textsf{\upshape{dbf}}}
\newcommand{\den}{{{\delta}}}
\newcommand{\load}{\ell}
\newcommand{\compress}{{{\gamma}}}
\newcommand{\feature}{{{\Omega}}}
\newcommand{\opt}{\textsf{\upshape{OPT}}}
\newcommand{\summation}{\textrm{sum}}
\newcommand{\maximum}{\textrm{max}}
\newcommand{\minimum}{\textrm{min}} 


\newcommand{\dendesum}{{{\omega}}} 
\newcommand{\dendemax}{{{\varpi}}} 
\newcommand{\pasum}{{{\lambda}}}
\newcommand{\pamax}{{{\rho}}}
\newcommand{\node}{{{\upsilon}}}

==> desegmentation.tex <==
\subsection{Vertex Reassembling}\label{ss:runtime}

 \begin{figure}[!t]
\centering
\subfigure[Before reassembling.]{\includegraphics[width=3.5in]{before.jpg}}
\subfigure[After reassembling.]{\includegraphics[width=3.5in]{after.jpg}}
\caption{\xuadd{Reassembling of the decomposed task.}}
\label{fig.reconstruction}
\end{figure}

The above segmentation procedure may split a vertex into several parts and each of them
is assigned to a different segment. However, at runtime we do \emph{not} need to schedule them individually.
Instead, we will treat the entire vertex as a scheduling entity.
Recall that initially the segments are divided according to the earliest ready time $\start(v)$ of vertices (which are also the latest finish time of vertices).
As the segments are \enquote{sketched} in the step of laxity distribution, we will adjust these time constraints
accordingly and use them as the vertex release time and deadlines.

Figure \ref{fig.reconstruction}-(a) shows the results after the segmentation and laxity distribution steps in the above subsections,
in which both $v_2$ and $v_4$ are split into two parts. The dashed box denotes the part that originally belongs to $v_2$'s
lifetime window before being split. Figure \ref{fig.reconstruction}-(b) shows that
different parts of a vertex are reassembled  with their release times and deadlines (which have been adjusted when the
segment is \enquote{sketched} in the laxity distribution step).

Finally, load and maximal density bounds of segments are still applicable to the decomposed task after vertex reassembling:
\begin{lemma}\label{l:bound}
For a decomposed task  $\tau_i$ (after vertex reassembling) we have
$\load_i \leq \hat{\dendesum}$,
and $\forall v  \in \tau_i: \den(v) \leq \hat{\dendemax}$.
\end{lemma}
The proof of Lemma \ref{l:bound} follows the same idea as Theorem 1 in \cite{saifullah2014parallel}, and thus
omitted here.

%\xuadd{After reconstruction the task $\tau_i$ in Fig.\ref{fig1} is shown in Fig.\ref{fig.reconstruction}. }
%
%At runtime, each vertex is treated as an independent sporadic task, and all the vertices (from different tasks)
%are scheduled by Global EDF algorithm.


==> diagram.tex <==
\subsection{Segmentation}\label{ss:segmentation-first}

To divide a task into segments, we first construct the \emph{timing diagram} of task $\tau_i$,
%\todo{Note that the timing diagram construction method in this paper is different from
%and introduces less pessimism than those in previous decomposition-based scheduling of parallel tasks \cite{,,}.
%We will compare them and outline the advantage of our method at the end of section \ref{s:decomp}.}
%
%
which defines the \emph{earliest ready time} of each vertex $v$, denoted by $\start(v)$,
and the \emph{latest finish time} of $v$, denoted by $\finish(v)$, assuming that
$\tau_i$ executes exclusively on sufficiently many processors and all the workload of $\tau_i$
must be finished within $L_i$.


Assuming $\tau_i$ releases an instance at time $0$, then for each vertex $v$, $\start(v)$ is computed by
\begin{equation*}
\start(v) = \left \{
\begin{array}{cl}
0,                                        & ~~\precde(v) = \emptyset \\
\displaystyle \max_{u \in \precde(v)}\{c(u) +  \start(u) \}, & ~~\textrm{otherwise}
\end{array}\right.
\end{equation*}
%\[
%\max_{\node_i^k \in \precde(\node_i^j)}\left\{~ C_i^j ~+~  \textrm{earliest ready time of }\node_i^k ~ \right\},
%\]
where $\precde(v)$ is the set of predecessors of $v$, and $\finish(v)$ is computed by
\begin{equation*}
\finish(v) = \left \{
\begin{array}{cl}
L_i,                        & ~~\success(v) = \emptyset \\
\displaystyle \min_{u \in \success(v)}\{ \start(u) \}, & ~~\textrm{otherwise}
\end{array}\right.
\end{equation*}
where $\success(v)$ is the set of successors of $v$.
In this way, all the dependency constraints of a task are preserved if each vertex executes in \emph{lifetime window} $[\start(v) , \finish(v) ]$.
Figure \ref{fig2} shows the timing diagram of the example task in Figure \ref{fig1}.


%\todo{For example ...}
%
%\todo{rename the vertices, rephrase the following paragraph}

%We can observed that $\node_i^2$ and $\node_i^4$ have 3 and 8 unit time of inherent laxity, respectively. This representation could be a more accurately reflection of the dependencies of tasks with out introducing any additional constraints.

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{fig2b.jpg}
\caption{\xuadd{Timing diagram of the task example in Figure \ref{fig1}. The
earliest ready time and latest finish times are marked as upper and lower arrows.}}
\label{fig2}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{fig2b-seg.jpg}
\caption{\xuadd{Segmentation of the task example in Figure \ref{fig1}. }}
\label{fig2-seg}
\end{figure}



==> experiments.tex <==
\section{Evaluations}
In this section, we evaluate our proposed decomposition algorithm by experiments. In particular, we will compare the
acceptance ratio of our proposed algorithm and schedulability test, denoted by $\DOUR$ with the state-of-the-art of all the three
paradigms:

\begin{itemize}
\item Decomposition-based scheduling: We compare with the EDF-based
scheduling algorithm and analysis techniques developed in \cite{saifullah2014parallel},
denoted by $\DSAI$.
\item Global scheduling: We compare with the following analysis methods in this category:
\begin{itemize}
\item The schedulability test based on workload analysis for GEDF in \cite{baruah2014improved}, denoted by $\GBAR$.
\item The schedulability test based on capacity augmentation bounds for GEDF in \cite{li2014analysis}, denoted by $\GLI$.
\item The schedulability test based on response time analysis for GEDF in \cite{melani2015response}, denoted by $\GMEL$.
Note that $\GMEL$ was developed for a more general conditional DAG task mode. However, it can be directly
applied to the DAG model of this paper, which is a special case of the one in \cite{melani2015response}.
\end{itemize}

\item Federated scheduling: We compare with the schedulability test based on capacity augmentation bounds in \cite{li2014analysis},
denoted by $\FLI$.
\end{itemize}
Other methods not included in our comparison are either
theoretically dominated or shown to be significantly
outperformed (with empirical evaluations) by
one of the above listed methods.
%for two main purposes: First, we compare out proposed algorithm with other schedulability test. Second, we would like to find out what factors have an impact on the efficiency of scheduling.

 \begin{figure}[!t]
\centering
\includegraphics[width=3.2in]{ratio_on_utilization.pdf}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Comparison with different normalized total utilization. $m=8$, $n=5$ and $p=0.01$.}
\label{fig6}
\end{figure}


\begin{figure}[!t]
\centering
\includegraphics[width=3.2in]{ratio_on_processors.pdf}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Comparison with different number of processors. $\util_{\summation}=3$, $n=5$ and $p=0.01$.}
\label{fig7}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=3.2in]{ratio_on_tasks.pdf}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{Comparison with different $p$. $\util_{\summation}=3$, $m=8$ and $n=5$.}
\label{fig8}
\end{figure}



The task sets are generated using the Erd\"{o}s-R\'{e}nyi method $G(n_i , p)$ \cite{cordeiro2010random}.
For each task, the number of vertices is randomly chosen in the range $[50, 250]$ and the worst-case execution time of each vertex
is randomly picked in the range $[50, 100]$, and a valid period is generated according to its target utilization.
For each possible edge we generate a random value in the range $[0, 1]$
and add the edge to the graph only if the generated value is less than a predefined threshold $p$.
In general the critical path of a DAG generated using the Erd\"{o}s-R\'{e}nyi method becomes longer as $p$ increases, which makes the task more sequential.
We compare the \emph{acceptance ratio} of each of the methods. The acceptance
ratio is the ratio between the number of task sets deemed to be schedulable by a method and
the total number of task sets that participate in the experiment (with a specific
parameter configuration).



    Figure \ref{fig6} shows the acceptance ratios of different methods under different \emph{normalized utilization} ($U_{\summation} / m$) of the task sets, with $m=8$, $n=5$ and $p=0.01$. The experiment results show that our method $\DOUR$ clearly outperforms all the others. The breakdown normalized utilization of $\DOUR$ is around $0.6$, while is below $0.5$ for all the others.


%    ADA could even schedule some task sets with 60\% utilization while the one in \cite{melani2015response} is nearly 50\%. The test based on capacity augmentation bound in \cite{li2014analysis} could only obtain nearly 40\% utilization because the total utilization is upper bounded by $\frac{3+\sqrt{5}}{2}$.

    Figure \ref{fig7} shows acceptance ratios with different number of processors, with a fixed number of tasks in each set $n=5$, $p=0.01$
    and the total utilization $U_{\summation}$ of each task set being $3$. Similar to Figure \ref{fig6},
    $p$ is also randomly chosen from the its candidate set. Since the total workload is fixed now, it becomes easier to successfully schedule
    a task set with more processors. The experiment results show that $\DOUR$ requires less processors than all the others to make
    the task sets to be schedulable.

    Figure \ref{fig8} shows acceptance ratios under different $p$ (which determines the parallelism of tasks), with $U_{\summation} = 3$, $n=5$
    and $m=8$. We can observe that for all the methods, the schedulability is better for tasks with higher parallelism.
    This is because, for a task with fixed total amount of workload, a more parallel structure in general leads to a shorter critical path,
    and thus more laxity, which is beneficial to schedulability. Since the trend of methods of different paradigms is the same,
    we can conclude that the effect of parallelism to schedulability is inherent to the parallel task model, but not the
    caused by any of these particular scheduling methods.
    Figure \ref{fig8} shows the superiority of our method $\DOUR$ over others with different parallelism degrees.
    Note that in this group of experiments, no task set is deemed schedulable by $\DSAI$ or $\GBAR$. In order to reflect the differences of various value of $p$ among the approaches with better acceptance ratio, we choose task sets with relatively high utilization. This is consistent with the results in the previous two figures. For example,
    the parameter setting of task sets with $p=0.01$ in Figure \ref{fig8} is the same as task sets with $m=8$ in Figure \ref{fig7}.
    The corresponding acceptance ratios of each method with this particular setting are basically the same in two figures.


    In summary, $\DOUR$ consistently outperforms other methods in all the above experiments with varying parameters in different dimensions.


%    \todo{...it is not surprising that we outperform ..., but we are also better
%    than the response time analysis method which requires... move this into a summary part? }
    %
%
%    For various values of $p$, we find that ADA is slightly harder to schedule sequential tasks than more parallel tasks while the total utilization and the number of tasks keep the same as shown in Fig.\ref{fig8}. This is because maximum of $\compress_{i}$ increase as the task become more sequential while the utilization keeps the same.The trends are the similar in other tests.
%
%    We also evaluate the schedulability when the task number varied in [1,20] while $m=8$ and the total utilization of 3. The result shows that the schedulablility of ADA and the test in both \cite{melani2015response}\cite{li2014analysis} keep stable while the number of tasks is more than a certain number(5, 6 and 7 perspectively). The schedulability in \cite{baruah2014improved} has a light improvement while the utilization of single task decreases.However, the differences of all of the 4 tests are very small while processors are not fully loaded hence that we didn't show the picture.
%
% \begin{figure}[!t]
%\centering
%\includegraphics[width=3.2in]{speed_up_of_processors.pdf}
%% where an .eps filename suffix will be assumed under latex,
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%% via \DeclareGraphicsExtensions.
%\caption{The speed up factor of ADA as a function of $m$ .}
%\label{fig10}
%\end{figure}
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=3.2in]{speed_up_of_P.pdf}
%% where an .eps filename suffix will be assumed under latex,
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%% via \DeclareGraphicsExtensions.
%\caption{The speed up factor of ADA as a function of $p$.}
%\label{fig11}
%\end{figure}
%
%We also evaluate the speed up factor of ADA.From equation 1, 2, two preconditions must be hold if a task set is schedulable: the total utilization must be smaller than m and the longest chain $L_i$ must be not greater than deadline $D_i$.Therefore we make the processors fully loaded by task set to evaluate the speed up factor which means for any number of $m$ we generated the task set whose total utilization is exactly $m$.
%
%In all our experiments, the maximum of the speed up factors is 2.2 and 85\% of the speed up factors in all task sets are below 2 which is much tighter than $\frac{3+\sqrt{5}}{2}$. Fig.\ref{fig10} shows that the speed up factor increase as the number of processors increase. This is because the maximum utilization of a single task increases as the number of processors increases such that the maximum of $\compress_i$ could potentially increases which may introduce a failure of the schedulability test. Fig.\ref{fig11} demonstrate the speed up factor of various values of $p$. The results shows that the speed up factor first decrease and then increase. This is because the length of critical path decreases as $p$ increases by the original Erd\"{o}s-R\'{e}nyi method. As we generate several more edges to make the DAG weak connected, the length of critical path first decreases and then increases again as $p$ increases.As we explain before the schedulability will be reduced as the length of critical path increases while all other parameters keep the same.
%
%The results of the experiments demonstrate that our schedulablility test is much tighter and more flexible than the existed ones. 

==> guan-decompose.tex <==
\section{General Schedulability Tests}

A density-based schedulability test condition is known for
traditional sequential sporadic task sets :
\todo{add the gossens 2003 reference}
\begin{theorem}\cite{baruah2007techniques,goossens2003}
Given a sequence sporadic task set, let $\den_{sum}$ denote
the total density of the task set, and $\den_{max}$ denote the
maximal density among all tasks. The task set is schedulable by global EDF scheduling
on $m$ processors if  if it satisfies:
\[
\den_{\summation} \leq m - (m-1) \den_{\maximum}
\]
\end{theorem}
A similar schedulability
test condition can be obtained for our parallel task systems, based on load instead of density:
\begin{theorem}\label{t:general-test-1}
A parallel task system is schedulable by global EDF scheduling
on $m$ processors if it satisfies:
\begin{equation}\label{e:general-test-1}
\load_{\summation} \leq m - (m-1) \den_{\maximum}
\end{equation}
\end{theorem}
where $\load_{\summation}$ is the sum of load of all tasks, and $\den_{\maximum}$
is the maximal density among all nodes of all tasks, i.e.,
\[
\den_{\maximum} = \max_{\tau_i \in \Gamma}\left\{\max_{v_i^j \in \tau_i} \{\den_i^j \} \right \}
\]


Theorem \ref{t:general-test-1} has been presented and used as the basis in previous work
\cite{,,} on decomposition-based global EDF scheduling\footnote{\todo{they use load and density
interchangeably...}}. However, in those papers,
this theorem is only claimed following informal arguments, but never been strictly proved.
Strictly speaking, the arguments presented in \cite{,,} is not very strict
(but the result is correct). We will discuss this issue and provide a strict proof for Theorem \ref{t:general-test-1} in the Appendix.


The schedulability test (\ref{e:general-test-1})
 does not depend on any particular
task decomposition strategy. However, different decomposition strategies
may lead to different values of $\load_{sum}$ and $\load_{max}$.
A parallel task set may pass the schedulability test (\ref{e:general-test-1})
with a \enquote{good} decomposition strategy,
but fail the test with a \enquote{bad} decomposition strategy.
For example, \todo{need an example}
Therefore, our target is to design good decomposition strategies, in order to
increase the chance for a task set to deemed to be schedulable.

\todo{we want suboptimal decomposition, bla bla bla}







==> guan-model.tex <==
\section{Preliminary}\label{s:pre}

\subsection{Task Model}\label{ss:task-model}

%\todo{Task, subtask, instance, job ...}
We consider the scheduling problem of a task set $\tau$ consisting of $n$ periodic tasks $\{\tau_1,\tau_2,...,\tau_n\}$,
 executed on $m$ identical processors.
Each task is represented by a DAG, which is released periodically with a period $T_i$.
We assume all tasks to be implicit-deadline, i.e., the workload released by a task at time $t$ must
be finished by the next release time $t+T_i$.


Each task $\tau_i$ is a  directed acyclic graph (DAG) consisting of several vertices and edges connecting them.
With a slight abuse of notations, we sometimes also use $\tau_i$ to denote the set of vertices in the corresponding DAG,
A vertex $v \in \tau_i$ has a worst-case execution time  $c(v)$.
Edges represent dependencies among vertices. A directed edge from vertex $v$ to $u$ means that $u$ can only be executed after $v$ is finished.
In this case, $v$ is a \emph{predecessor} of $u$, while $u$ is a \emph{successor} of $v$.
%\todo{The number of vertices can may simultaneously execute is called the parallelism of the task. Since there are only $m$ processors,
%we restrict ourself to task graphs with parallelism of at most $m$\footnote{A tasks with parallelism larger than $m$ can be transformed
%to one with  parallelism at most $m$ by adding some edges into the original task graph.}}.




The total execution time of all vertices of task $\tau_i$ is denoted by $C_i = \sum_{v \in \tau_i} c(v)$.
The utilization $U_i$ of a task $\tau_i$ and the total utilization $U_{\summation}$ of the task set $\tau$
are defined as follows
\begin{equation}
\util_i= \frac{C_i}{T_i}, ~~\util_{\summation}(\tau)=\sum_{\tau_i \in \tau} U_i
\end{equation}

$L_i$ denotes the sum of $c(v)$ of each vertex $v$ on the longest chain (also called the critical path) of task $\tau_i$, i.e., the execution time of the task $\tau_i$ to be exclusively executed on infinite number of cores. The \emph{laxity} of task $\tau_i$ is $T_i - L_i$.
We use $\compress_i$ to denote the \emph{elasticity} of task $\tau_i$, which is defined as
\[
\compress_i =\frac{L_i}{T_i}
\]
Figure \ref{fig1} shows a DAG task example with $8$ vertices. The utilization of this task
is $C_i/T_i = 30/25$, the laxity is $T_i - L_i = 10$ and the elasticity is $L_i/T_i = 15/25$.





Apparently if a task set $\tau$ is schedulable on $m$ processors the following necessary conditions must hold:
% conference papers do not normally have an appendix
\begin{equation}
\forall \tau_i \in \tau: L_i\leq{T_i},  ~\textrm{and}~ \sum_{\tau_i \in \tau}U_i \leq {m};
\label{eq1}
\end{equation}

\subsection{Task Decomposition}\label{ss:decomposition}
The target of task decomposition is to assign an artificial release time and deadline to each vertex
(relative to the release time of the entire task), such that the dependencies among different vertices are automatically guaranteed as long as each individual vertex respects its own release time and deadline constraints.



We use $d(v)$ to denote the relative deadline of a vertex $v$ in a decomposed task, and the \emph{density} of this vertex is
\[
\den(v) = \frac{c(v)}{d(v)}
\]

We define the demand bound function $\dbf_i(t)$ of a decomposed task ${\tau_i}$
as the maximal accumulative workload over a time interval of length $t$, released by ${\tau_i}$'s subtask instances which have both release time and deadline
in this time interval.
The \emph{load} of a decomposed task $\tau$ is defined as
\begin{equation}\label{e:load}
\load_i = \max_{t>0}\left( \frac{\dbf_i(t)}{t} \right)
\end{equation}

%\todo{give values of dbf and load of the example ... }
The above defined demand bound function and load are natural generalizations
of their correspondence for sequential sporadic tasks \cite{baruah90edf}.
In practise, both $\dbf_i(t)$ and $\load_i$ can be calculated in polynomial time. However, their actual calculation methods are not of our interests
since they are merely used as auxiliary concepts in this paper and
our scheduling and analysis techniques do not really need to compute them.

\begin{figure}[!t]
\centering
\includegraphics[width=2.4in]{fig1.jpg}
% where an .eps filename suffix will be assumed under latex,
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
\caption{\xuadd{A DAG task example.}}
\label{fig1}
\end{figure}

\forget{
\begin{table}\label{t:symbols}
\begin{tabular}{|c|c|c|}
	\hline Notation & Definition & Remark \\
	\hline $\den_i$ & $ C_i/D_i$ & density of task $\tau_i$ \\
	\hline $\compress_i$  & $ L_i/D_i$ & compressibleness of task $\tau_i$\\
	\hline $\load_i$  & (\ref{e:load}) in Section \ref{ss:decomposition} & load of a decomposed task $\tau_i$\\
	\hline $\feature_i$  &  &  \\
	\hline
\end{tabular}
\caption{Important symbols.}
\end{table}
}

\subsection{A Known Schedulability Test Condition}

After decomposition, the following
condition can be applied to check the schedulability of the task set \cite{saifullah2013multi,qamhieh2014stretching}:
\begin{theorem}\label{t:general-test-1}
A decomposed task set $\tau$ is schedulable by global EDF scheduling
on $m$ processors if it satisfies:
\begin{equation}\label{e:general-test-1}
\load_{\summation} \leq m - (m-1) \den_{\maximum}
\end{equation}
where $\load_{\summation}$ is the sum of load of all tasks, and $\den_{\maximum}$
is the maximal density among all vertices of all tasks:
\[
\load_{\summation} = \sum_{\tau_i \in \tau} \load_i , ~~ \den_{\maximum} = \max_{\tau_i \in \tau}\left\{\max_{v \in \tau_i} \{\den(v) \} \right \}
\]
\end{theorem}

The schedulability test in Theorem \ref{t:general-test-1} is the base of
previous work on decomposition-based global EDF scheduling of parallel tasks \cite{saifullah2013multi,qamhieh2014stretching}.
This schedulability test is independent on the specific
task decomposition strategy in use. However, different decomposition strategies
may lead to different values of $\load_{\summation} $ and $\den_{\maximum}$.
A parallel task set may pass the schedulability test (\ref{e:general-test-1})
with one decomposition strategy,
but fail with another.
Therefore, the target of this paper is to design good decomposition strategies, to minimize both
$\load_{\summation}$ and $\den_{\maximum}$, and thus increase
the chance for a task set to be deemed schedulable.



%Theorem \ref{t:general-test-1} has been presented and used as the basis in previous work
%\cite{,,} on decomposition-based global EDF scheduling\footnote{\todo{they use load and density
%interchangeably...}}. However, in those papers,
%this theorem is only claimed following informal arguments, but never been strictly proved.
%Strictly speaking, the arguments presented in \cite{,,} is not very strict
%(but the result is correct). We will discuss this issue and provide a strict proof for Theorem \ref{t:general-test-1} in the Appendix.








==> laxity.tex <==
\subsection{Laxity Distribution}\label{ss:laxity}
Next we distribute the total laxity $T_i - L_i$
of the task to each individual segment.
In other words, we will \enquote{stretch} the segments such that
the total length of all segments becomes from $L_i$ to $T_i$.
Intuitively,
the purpose of our laxity assignment strategy is to distribute the laxity
in a balanced manner to avoid any of the segments to cause an
outstanding workload burst.


We use $d(s^x)$ to denote the length of segment $s^x$ after laxity distribution,
and thus $d(s^x) - e(s^x)$ is the amount of laxity given to this segment
(recall that $e(s^x)$ is the length of the segment before the laxity assignment).
We enforce that each vertex in $s^x$ (or the part of a vertex assigned to this segment in case it is split) must finish execution by the end of this segment.
Therefore, $d(s^x)$ can be viewed as the common relative deadline of vertices (or parts of some vertices) in $s^x$.
We define \emph{load} caused by workload assigned to a segment.
\begin{define}
The \emph{load} of a segment is defined as
\begin{equation}
\dendesum(s^x) = \frac{c(s^x)}{d(s^x)}
\label{eq6}
\end{equation}
and we use $\hat{\dendesum}$ to denote the maximal load among all segments of task $\tau_i$:
\[
\hat{\dendesum} = \max_{x=1}^X \{ \dendesum(s^x) \}
\]
\end{define}
Moreover, we define the \emph{density} of a segment as
\begin{define}
The \emph{density} of segment $s^x$ is
\begin{equation}
  \dendemax(s^x)=\frac{e(s^x)}{d(s^x)}
\label{eq7}
\end{equation}
and we use $\hat{\dendemax}$ to denote the maximal density among all segments of task $\tau_i$:
\[
\hat{\dendemax} = \max_{x=1}^X \{ \dendemax(s^x) \}
\]
\end{define}

According to the schedulability test condition (\ref{e:general-test-1}) in Theorem \ref{t:general-test-1}, to improve the schedulability
of the task set, we should minimize both the load and the maximal density among all the vertices for each task.
As will be seen later in Section \ref{ss:runtime} (known from \cite{saifullah2014parallel}),
the load of a task is actually bounded by $\hat{\dendesum}$
and the maximal density of a task is bounded by $\hat{\dendemax}$. Therefore, in the laxity distribution step
we will try to minimize both $\hat{\dendesum}$ and $\hat{\dendemax}$.


However, in general minimizing $\hat{\dendesum}$ and $\hat{\dendemax}$ may contradict each other.
Recall that we classify the segments into two types: light segments and heavy segments. Intuitively,
we should give more laxity to heavy segments since, otherwise they will cause a large $\dendesum(s^x)$.
However, on the other hand, if we give too much laxity to heavy segments, and thus
do not give enough laxity to light segments,
$\hat{\dendemax}$ will become very large, which also hurts the schedulability.
Therefore, the challenge is how to find a systematical laxity distribution strategy to make a good balance
between $\hat{\dendesum}$ and $\hat{\dendemax}$. In the following we present our laxity distribution strategy which unifies the minimization of $\hat{\dendesum}$ and $\hat{\dendemax}$.


%
%
%\todo{our target is ... }
%In order to get a better schedulability we need to make the load and the maximum sequential density of segment bounded as small as possible.Suppose that there are $m$ segments in $\light_i$ and n segments in $\heavy_i$. Therefore, for a heavy segment $s_i^h$($1\leq{h}\leq{m}$), it need to be assigned more laxity to decrease $\dendesum_i^h$  while the $\dendemax_i^h$ will also be decreased due to more laxity assignment. When the heavy segments get more laxity, a light segment $s_i^l$($1\leq{l}\leq{n}$) may get less laxity such that both the $\dendesum_i^l$ and $\dendemax_i^l$ potentially increase.
%
%For each heavy segment $s_i^h$, we can make $\dendesum_i^h$ equal to a threshold, and then obtain the upper bound $\hat{\dendemax_i^{\heavy}}$ due to $\dendesum_i^h$ is lower bounded by $\frac{C_i}{L_i}$. If we make a threshold to $\dendemax_i^h$, the load  in all heavy segments may still be infinity due to the load of a heavy segment is greater than $\frac{C_i}{L_i}$ and is upper bounded by $\infty$, such that we can not make the upper bound of the load.
%  For each light segment $s_i^l$, we can make $\dendemax_i^l$ equal to a threshold, and then obtain the corresponding upper bound $\hat{\dendesum_i^{\light}}$ due to their densities are upper bounded by $\frac{C_i}{L_i}$. We deal with both heavy segments and light segments at the same time, then for task $\tau_i$, we could get  $\hat{\dendesum_i}$ and $\hat{\dendemax_i}$. Fig.\ref{fig3} indicates the principle of the task decomposition.

Our laxity distribution strategy is based on the following two rules:

\begin{itemize}
\item  \textbf{Rule 1}: for each heavy segment $s^h$,  we give laxity to it so that
\vspace{-2mm}
\begin{equation}
\dendesum(s^h) =\frac{c(s^h)}{d(s^h)}=\pasum \util_{i}
\label{eq.deadlineh}
\end{equation}

\item \textbf{Rule 2}: for each light segment $s^l$, we give it laxity to it so that
\vspace{-2mm}
\begin{equation}
\dendemax(s^l) =\frac{e(s^l)}{d(s^l)}=\pamax\compress_{i}
\label{eq.deadlinel}
\end{equation}
\end{itemize}
where $\pasum$ and $\pamax$ are two positive factors that will be decided later in this subsection.
In the following we show that although the above two rules only control the
load of a heavy segment and the density of a light segment, actually the density of
the heavy segment and the load of the light segment can also be correspondingly bounded,
and thereby the maximal load and maximal density among all segments are bounded.

\begin{lemma}\label{l:unify}
The maximal density of any segment (either heavy or light) of $\tau_i$ is upper bounded by
\begin{equation}\label{e:unift-density}
\hat{\dendemax} \leq \max(\pasum, \pamax)  \cdot  \compress_{i}
\end{equation}
and the maximum load of any segment (either heavy or light) of $\tau_i$ is upper bounded by
\begin{equation}\label{e:unift-load}
\hat{\dendesum}  \leq \max(\pasum , \pamax ) \cdot \util_{i}
\end{equation}
\end{lemma}
\begin{proof}
We first prove (\ref{e:unift-density}) by bounding the density of an arbitrary \emph{heavy} segment $s^h$:
\[
 \dendemax(s^h)=\frac{e(s^h)}{d(s^h)}=  \frac{c(s^h)}{d(s^h)} \cdot \frac{e(s^h)}{c(s^h)} =    \pasum\util_{i} \frac{e(s^h)}{c(s^h)}
\]
 A heavy segment $s^h$ satisfies $\frac{c(s^h)}{e(s^h)} >{\frac{C_i}{L_i}}$, i.e., $\frac{e(s^h)}{c(s^h)} <{\frac{L_i}{C_i}}$, so we have
\begin{equation*}
\dendemax(s^h) = \pasum\util_{i} \frac{e(s^h)}{c(s^h)}
< \pasum\util_{i}\frac{L_i}{C_i}
= \pasum\frac{C_i}{T_i}\frac{L_i}{C_i}=\pasum\frac{L_i}{T_i} =\pasum\compress_{i}
\label{eq9}
\end{equation*}
Combining this with (\ref{eq.deadlinel}) proves (\ref{e:unift-density}).

Then we prove (\ref{e:unift-load}) by bounding the load of an arbitrary \emph{light} segment $s^l$.

%We define $\hat{\dendesum_i^H}$ as an upper bound of $\dendesum_i^h$ during all heavy segments and $\hat{\dendesum_i^L}$ for light segments. Similar,We define $\hat{\dendemax_i^H}$as an upper bound of $\dendemax_i^h$ in all heavy segments and $\hat{\dendemax_i^L}$ for light segments. Therefore, for all segments in $\heavy_i$, we have $\hat{\dendesum_i^H}=\pasum\den_{i}$ while $\hat{\dendemax_i^H}=\pasum\compress_{i}$.


%  For each light segment $s_i^l$, after the laxity assignment, we have $\dendesum_i^l$ to be:

\begin{equation*}
  \dendesum(s^l)=\frac{c(s^l)}{d(s^l)} = \frac{e(s^l)}{d(s^l)} \cdot \frac{c(s^l)}{e(s^l)} =\pamax \compress_{i} \frac{c(s^l)}{e(s^l)}
\label{eq10}
\end{equation*}
Since a light segment satisfies $\frac{c(s^l)}{e(s^l)}\leq\frac{C_i}{L_i}$, we have
\begin{equation*}
  \dendesum(s^l) = \pamax \compress_{i} \frac{c(s^l)}{e(s^l)} = \pamax \frac{L_i}{T_i} \frac{c(s^l)}{e(s^l)} \leq  \pamax \frac{L_i}{T_i} \frac{C_i}{L_i}
  = \pamax  \frac{C_i}{T_i} = \pamax\util_{i}
\label{eq12}
\end{equation*}
Combining this with (\ref{eq.deadlineh}) proves (\ref{e:unift-load}).
\end{proof}





From Lemma \ref{l:unify} we can see that both $\hat{\dendemax}$ and $\hat{\dendesum}$
depend on $\max(\pasum , \pamax)$. Therefore, the minimization of $\hat{\dendemax}$ and $\hat{\dendesum}$
is now unified --  we want to minimize $\max(\pasum , \pamax)$.
The following lemma gives the relation between $\pasum$ and $\pamax$:

\begin{lemma}\label{l:sum}
Given a decomposed task $\tau_i$, the following relation between $\pasum$ and $\pamax$ holds:
\begin{equation}\label{e:sum}
1  = \frac{C_i^{\heavy}}{\pasum C_i} + \frac{L_i^{\light} }{\pamax L_i}
\end{equation}
where
\begin{equation*}
C_i^{\heavy}  = \sum_{s^x \in \heavy_i} c(s^x), ~~  L_i^{\light}  = \sum_{s^x \in \light_i} e(s^x)
\end{equation*}
\end{lemma}
\begin{proof}
By (\ref{eq.deadlineh}) we know for each heavy segment $s^h$:
\begin{equation*}
d(s^h)=\frac{c(s^h)T_i}{\pasum{C_i}}
\label{eq15}
\end{equation*}
and by (\ref{eq.deadlinel}) we know for each light segment $s^l$:
\begin{equation*}
d(s^l)= \frac{e(s^l)T_i}{\pamax{L_i}}
\label{eq16}
\end{equation*}
Hence we have
%\begin{equation}
%D_i = \sum_{s^h \in \heavy}d(s^h) + \sum_{s^l \in \light}d(s^l) = \frac{C_i^{\heavy}D_i}{\pasum C_i} + \frac{L_i^{\light}D_i }{\pamax L_i}
%\label{eq20}
%\end{equation}
\begin{equation*}
T_i = \sum_{s^h \in \heavy}d(s^h) + \sum_{s^l \in \light}d(s^l) = \frac{C_i^{\heavy}T_i}{\pasum C_i} + \frac{L_i^{\light}T_i }{\pamax L_i}
\label{eq20}
\end{equation*}
which proves (\ref{e:sum}) by removing $T_i$ from both sides of the equation.
\end{proof}

By Lemma \ref{l:sum} we know $\pasum$ and $\pamax$ are inversely proportional to each other. Therefore, $\max(\pasum , \pamax)$
is minimized when $\pasum = \pamax$, and according to (\ref{e:sum}) this results in
\[
\pasum = \pamax = \frac{C_i^{\heavy}}{C_i} + \frac{L_i^{\light}}{L_i}
\]
We define this value as the \emph{structure characteristic value} of a decomposed task, denoted by $\feature_i$:
\begin{define}
The \emph{structure characteristic value} of a decomposed task $\tau_i$ is defined as
\begin{equation}
\feature_i = \frac{C_i^{\heavy}}{C_i} + \frac{L_i^{\light}}{L_i}
\end{equation}
\end{define}
Then the bounds in Lemma \ref{l:unify} can be rewritten as
\begin{equation}\label{e:rewrite}
\hat{\dendesum} \leq \feature_i\util_{i}, ~~ \hat{\dendemax}\leq \feature_i\compress_{i}
\end{equation}
To minimize these upper bounds of both $\hat{\dendesum}$ and $\hat{\dendemax}$, we shall minimize $\feature_i$.
We observe that $\feature_i$ depends on $C_i^{\heavy}$ and $L_i^{\light}$ (while $C_i$ and $L_i$ are fixed constants
for a given task $\tau_i$). Both $C_i^{\heavy}$ and $L_i^{\light}$ are decided in the segmentation step.
Recall that in Section \ref{ss:segmentation-first} we left it open about how to do the segmentation, i.e.,
how to assign the vertices to different segments. Now it becomes clear that the target of our segmentation
strategy is to minimize $\feature_i$. In the following we will introduce in detail our segmentation strategy
that leads to the minimal  $\feature_i$.

%
%\todo{move the following somewhere else ... }
%
% We denote $\tau_i^{''}$ to be the subtasks set after the decomposition on $\tau_i^{\infty}$. The laxity assignment of $\tau_i$ in Fig.\ref{fig1} is shown in Fig.\ref{fig4}.

%\begin{figure}[!t]
%\centering
%\includegraphics[width=3in]{fig4b.jpg}
%\caption{\xuadd{Task decomposition on $\tau^{'}$.}}
%\label{fig4}
%\end{figure}







==> multiDAG.tex <==
\section{schedulability test}\label{s:multiDAG}
In this section, a schedulablity analysis is presented for a task set consists of several parallel DAG tasks which is scheduled on a given uniform multiprocessor platform. The schedulability analysis is based on the response time bound for single task. Additionally, we consider the interference on each task $\tau_i$ of all other tasks that may fall in the life window of $\tau_i$.

\begin{define}
The interference work $I_{i,k}$ is defined as the cumulative workload executed by task $\tau_i$ during the release time and finishing time of $\tau_k$.
\label{define:interference}
\end{define}


\begin{lemma}
Considering a task set $\tau$ is schedule upon a uniform m-processor platform $\platform$ by any work-conserving algorithm, an upper-bound of the response time of task $\tau_k$ is given by $\response_k$:
\begin{equation}
\response_k\leq\frac{C_k+L_k\platfeature(\platform)+\displaystyle\sum_{\forall_i\neq{k}}I_{i,k}}{S_m}
\label{eq:boundmulti}
\end{equation}
\label{l:schedulabilitytest}
\end{lemma}

\begin{proof}
	From equation \ref{eq:C=}, we can easily obtain that after add up all the interference work of other tasks:
	\[
	C_k+\displaystyle\sum_{\forall_i\neq{k}}I_{i,k}=\sum_{i=1}^{m}y_i\sumspeed_i
	\]
	Thus with \ref{eq:pluslambada} we have:
	\[
	y_m\sumspeed_m+\sum_{i=1}^{m-1}y_i\sumspeed_m\leq	C_k+L_k\platfeature(\platform)+\displaystyle\sum_{\forall_i\neq{k}}I_{i,k}
	\]
	\[
	\Rightarrow \response_k\sumspeed_m\leq{C_k+L_k\platfeature(\platform)+\displaystyle\sum_{\forall_i\neq{k}}I_{i,k}}
	\]
	Hence follow the lemma.
\end{proof}

\begin{lemma}
	An upper-bound on the workload of an interfering task $\tau_i$ in a window of length $t$ is given by:
	\[
	\Theta(t)=\lfloor{\frac{t+R_i-C_i/\sumspeed_m}{D_i}}\rfloor{C_i+}
	\]	
	\[
	\min(C_i,\sumspeed_m((t+R_i-C_i/\sumspeed_m)\mod{D_i}))
	\]
\end{lemma}

\begin{lemma}
	An upper-bound on the workload of an interfering task $\tau_i$ on task $tau_k$ with global EDF is given by:
	\[
	\Psi_{i,k}=\lfloor\frac{D_k}{D_i}\rfloor C_i+
	\]
	\[
	\min(C_i,\sumspeed_m\cdot\max(0, D_k\mod{D_i}-D_i+R_i))
	\]
\end{lemma}

\begin{theorem}
	Given a parallel task set scheduled on a m-processor uniform platform $\platform$, an upper-bound $R_{k}^{up}$ on the response time of a task $\tau_k$ can be derived by the fixed-point interaction of the following expression, starting with $R_{k}^{up}=\frac{L_k}{\speed_1}$
	
	\begin{equation}
	R_{k}^{up}\leftarrow\frac{C_k+L_k\platfeature(\platform)}{\sumspeed_m}+\frac{1}{\sumspeed_m}\sum_{\forall_i\neq{k}}I_{i,k}
	\label{eq:schedulability_test}
		\end{equation}
		when scheduled by global EDF:
		\[
		I_{i,k}=\min\{{\Theta(R_{k}^{up}),\Psi_{i,k}}\}
		\]
	  when scheduled by any other work-conserving algorithm, $I_{i,k}=\Theta(R_{k}^{up})$.
	  \label{th:test}
\end{theorem}

The schedulability of a parallel task sets consists of several tasks can be easily checked by using Theorem \ref{th:test}. At the beginning of the test, all bound are initially set to $R_{k}^{up}=\frac{L_k}{\sumspeed_m}$. Then \ref{eq:schedulability_test} is used to compute a response time of each task.The procedure continues until either (i) one of the response-time bounds exceeds the corresponding task deadline(return test failed), or (ii) no more update is possible(return success).
















==> optimal.tex <==
\section{Optimal Decomposition Strategy}

==> overview.tex <==
\section{New Decomposition Strategy}

This section introduces our new decomposition strategy, which
consists of two major steps: (i) segmentation and (ii) laxity distribution.
In the segmentation step, we divide the time window between two successive release times of $\tau_i$
(the length is $T_i$) into several \emph{segments},
and assign the workload of each vertex into these segments (a vertex may be split into several
parts and each part is assigned to a different segment, as will be introduced later).
In the laxity distribution step, the laxity $T_i - L_i$ of this task is distributed into
each segment, and thus given to the vertices in each segment accordingly.

The overall target of our decomposition strategy is to
make the load of each segment and maximal density of
its contained vertices to be as uniform as possible, and thus to minimize both
the load and the maximal density among all vertices.

In Section \ref{ss:segmentation-first}, we introduce the basic concepts of the segmentation phase.
Before presenting our new segmentation strategy, we first introduce our
laxity distribution strategy and related properties in Section \ref{ss:laxity}, after which
it will become clear how the segmentation strategy affects the schedulability of a task set.
Then we present our new segmentation strategy in Section \ref{ss:segmentation-second}.
{Finally, Section \ref{ss:runtime} shows how different parts of a vertex assigned
to different segments can be reassembled and scheduled as an entire entity at runtime,
without violating the desired workload and density bounds.}


%\begin{itemize}
%\item We first introduce the Timing Diagram of a task $\tau_i$, based on which
%\item
%\item
%\end{itemize}
%
%
%\begin{itemize}
%\item The idea is to assign the laxity $D_i-L_i$ to jobs. First to make
% the tightest sequence to make them looser.
%\item We will divide the whole sequence into segments, and assign laxity
%to each segment.
%\item The most important part is to decide the amount of laxity to be assigned to each segment.
%\end{itemize} 

==> schedulability.tex <==
\section{Analysis}

\subsection{Schedulability Test}
In the last section we presented how to transform the vertices in each task into sporadic tasks with artificial release time and deadlines.
In the following we show how to decide the schedulability of the resulting sporadic task system under GEDF scheduling.
The following theorem shows that we can directly use the structure characteristic values to test the schedulability of the task set.
%After the DAGs are decomposed into sequential constraint deadline subtasks, each node is assigned a release time, an execution time and a deadline, such that the scheduling of DAGs changes into the scheduling of sporadic sequential tasks. Now we can use the traditional multi-core scheduling algorithm to schedule them. In this section, we will discuss that the efficiency of the decomposition algorithm that we proposed by using GEDF algorithm.
%
%As we represent each DAG $\tau_i$ as $\tau_i^{\infty}$, all the dependencies were preserved. During the decomposition of $\tau_i^{\infty}$, we assigned the release time of each node to guarantee that each node can only start until all its parents are finished  while the execution time of each node and the whole deadline of $\tau_i^{sche}$ is the same as $\tau_i$. Hence if $\tau^{sche}$ is schedulable under a scheduling policy then $\tau$ must be also schedulable.
\begin{theorem}\label{theo4}
The resulting sporadic task set by decomposing the parallel task set $\tau$ is schedulable if it satisfies
\begin{equation}
m \geq \frac{\util_{\summation} - \compress_{\maximum}}
{\frac{1}{\feature_{\maximum} }- \compress_{\maximum}},
\label{eq25}
\end{equation}
where $\util_{\summation}$ is the total utilization of all tasks,  $\compress_{\maximum}$ and $\feature_{\maximum}$ is the maximal \emph{elasticity} and maximal \emph{structure characteristic value} among all tasks, respectively:
\[
\util_{\summation} = \sum_{\tau_i \in \tau} \util_i,~~\compress_{\maximum} = \max_{\tau_i \in \tau} \{\compress_i\},~~ \feature_{\maximum}
= \max_{\tau_i \in \tau} \{\feature_i\}
\]
\end{theorem}
%\todo{change $\load(\tau_i)$ to $\load_i$}
%!!!!!!!!!!!!!!!!
\begin{proof}
By Lemma \ref{l:bound} and (\ref{e:rewrite}) we have
\begin{equation}\label{eq:den}
\max_{v \in \tau_i} \{\den(v)\}\leq{\feature_{i}\compress_{i}}
\end{equation}
\begin{equation}\label{eq:load}
\load_i \leq {\feature_{i}\util_i}
\end{equation}
By (\ref{eq:den}) we have
\begin{align}
\den_{\maximum} & = \max_{\tau_i \in \tau} \left\{ \max_{v \in \tau_i} \{\den(v)\} \right\} \leq \max_{\tau_i \in \tau}\{ \feature_{i}\compress_{i} \} \nonumber \\
 & \leq
\max_{\tau_i \in \tau}\{ \feature_{i} \}\max_{\tau_i \in \tau}\{ \compress_{i} \} = \feature_{\maximum} \compress_{\maximum} \label{eq:den-max}
\end{align}
By (\ref{eq:load}) we have
\begin{equation}\label{eq:load-sum}
\load_{\summation} = \sum_{\tau_i \in \tau}  \load_i \leq  \sum_{\tau_i \in \tau}{\feature_{i}\util_i} \leq  \sum_{\tau_i \in \tau}{\feature_{\maximum}\util_i} = \feature_{\maximum} \util_{\summation}
\end{equation}
We can rewrite (\ref{eq25}) as
\[
\feature_{\maximum} \util_{\summation} \leq m - (m-{1})\feature_{\maximum} \compress_{\maximum}
\]
By applying (\ref{eq:den-max}) and (\ref{eq:load-sum}) to the above, we have
\[
\load_{\summation} \leq m - (m-1) \den_{\maximum}
\]
Therefore, by Theorem \ref{t:general-test-1} we know the resulting sporadic task set is schedulable.
\end{proof}


%!!!!!!!!!!!!!!!!
%We can apply condition \ref{eq30} as a sufficient schedulability test directly. In practical, by equation \ref{eq30}, for any given DAG task set $\tau$,we can provide that how many processors required to make all tasks to meet their deadline.

\subsection{Capacity Augmentation Bound}
%\todo{capacity augmentation, not speedup factor, check the previous part of the paper to make it consistent}
%
%\todo{add the definition of capacity augmentation bound, take from literatures}
%\xuadd{From ,}
Until now, all the task parameters are defined
on the basis of unit-speed processors. If we scale up/down the processor speed to $s$,
then each task parameter will be multiplied by $1/s$.


\begin{define}\cite{li2015global}
If on unit-speed processors, a task set has total utilization of at most $m$ and the critical path length of each task is smaller than its deadline,then a scheduler $S$ provides a \emph{capacity augmentation bound} of $s$ if it can schedule this task set on m processors of speed $s$.
\end{define}

Before proving the capacity augmentation bound of our algorithm, we generalize the test condition in Theorem \ref{t:general-test-1} to $s$-speed processors:
a task set is schedulable on $s$-speed processors if
\begin{equation}\label{e:s-speed}
\load_{\summation}^s \leq m - (m-1) \den_{\maximum}^s
\end{equation}
where $\load_{\summation}^s = \load_{\summation} / s$ and $\den_{\maximum}^s =  \den_{\maximum}/s$.
\begin{theorem}\label{t:capacity}
Our proposed decomposition-based scheduling algorithm has a capacity augmentation bound of $(2-\frac{1}{m}) \feature_{\maximum}$.
\end{theorem}
\begin{proof}
Assume $\tau$ is a task set with $\util_{\summation} \leq m$ and $\compress_{\maximum} \leq 1$.
Consider a $s$-speed processor platform, where $s = (2-\frac{1}{m})\feature_{\maximum}$.
By reusing (\ref{eq:den-max}) and (\ref{eq:load-sum}) in the proof of Theorem \ref{theo4} we have
\[
\dendemax_{\maximum}^{s} \leq \frac{\feature_{\maximum}\compress_{\maximum}}{s}
\leq  \frac{\feature_{\maximum}}{s}
\]
\[
\load_{\summation}^{s} \leq \frac{\feature_{\maximum} \util_{\summation}}{s} \leq \frac{\feature_{\maximum} m}{s}
\]
Combining them gives
\[
\load_{\summation}^{s} + (m-1) \dendemax_{\maximum}^{s} \leq \frac{\feature_{\maximum} m}{s} + (m-1) \frac{\feature_{\maximum}}{s} = \frac{(2m-1)\feature_{\maximum}}{s} = m
\]
which meets the condition (\ref{e:s-speed}) and thus the task set is schedulable on $s$-speed processors.
\end{proof}
%By the test condition (\ref{eq25}) in Theorem \ref{theo4} we can get the minimal number of processors needed to successfully schedule
%a task set by our algorithm. If setting the number of processors $m$ to be fixed, we can also get the minimal speed
%of the processors to make a task schedulable, by generalizing Theorem \ref{theo4}
%to $s$-speed processor platforms with similar proofs as above:


Now we take a closer look into the capacity augmentation bound $(2-\frac{1}{m}) \feature_{\maximum}$.
Recall the definition of the structure characteristic value of a task $\tau_{i}$:
\[
\feature_{i} = \frac{C_i^{\heavy}}{C_i} + \frac{L_i^{\light}}{L_i}
\]
where $C_i^{\heavy}$ and $L_i^{\light}$ are the results of the segmentation step. However, as stated in Theorem \ref{th:optimal-segmentation},
our segmentation algorithm yields the optimal (minimal) $\feature_i$, and thus the $\feature_i$ used in the capacity augmentation bound
of our scheduling algorithm is the minimum among all the possibilities. This minimal $\feature_i$ is indeed an
inherent feature of the task itself: the minimal $\feature_i$ of a task $\tau_i$ is only determined by the task
parameters, including its graph structure (although a polynomial-time algorithm is needed to actually compute it).


By the definition of $C_i^{\heavy}$ and $L_i^{\light}$, we know $\frac{C_i^{\heavy}}{C_i} \leq 1$ and $\frac{L_i^{\light}}{L_i} \leq 1$,
and $\frac{C_i^{\heavy}}{C_i}$ and $\frac{L_i^{\light}}{L_i}$ cannot equal to $1$ at the same time.
Therefore, we know $\feature_{\maximum}$ must be in the range of $[1,2)$, and thus the capacity augmentation bound
is in the range of $[2-\frac{1}{m}, 4-\frac{2}{m})$.

\forget{
The worst case value $4-\frac{2}{m}$ is the same
as in previous work \cite{??}.


Actually, we can further tighten the worst-case resource augmentation bound, as in the following theorem
\begin{theorem}
The worst-case capacity augmentation bound of our proposed decomposition-based scheduling algorithm is at most $(2-\frac{1}{m}) \feature_{\maximum}$.
\end{theorem}
\begin{proof}
By the definition of $\feature_i$ and $C_i^{\light} + C_i^{\heavy} = C_i$, we have
\begin{align*}
\feature_i & = \frac{C_i - C_i^{\light}}{C_i} + \frac{L_i^{\light}}{L_i} = 1 + \frac{L_i^{\light}}{L_i}-\frac{C_i^{\light}}{C_i} \nonumber\\
           & \leq 1 + \frac{L_i^{\light}}{L_i} - \frac{L_i^{\light}}{C_i} ~~(\because ~ C_i^{\light} \geq L_i^{\light} ) \nonumber\\
           & = 1 + L_i^{\light}\left( \frac{1}{L_i} - \frac{1}{C_i}\right)
\end{align*}
by which we have
\begin{equation}\label{e:feature-1}
L_i^{\light} \geq \frac{\feature_i - 1}{ \frac{1}{L_i} - \frac{1}{C_i}}
\end{equation}

on the other hand, by the definition of $\feature_i$ and $L_i^{\light} + L_i^{\heavy} = L_i$ we have
\begin{align*}
\feature_i =\frac{C_i^{\heavy}}{C_i} + \frac{L_i - L_i^{\heavy}}{L_i} =1 + \frac{C_i^{\heavy}}{C_i} - \frac{L_i^{\heavy}}{L_i} \nonumber \\
\end{align*}
Since the parallelism of each task is at most $m$, we know $C_i^{\heavy} \leq m L_i^{\heavy}$, so by the above we have
\begin{align*}
\feature_i    & \leq 1 + \frac{m \times L_i^{\heavy}}{C_i} - \frac{L_i^{\heavy}}{L_i} = 1 + L_i^{\heavy}\left( \frac{m}{C_i} - \frac{1}{L_i}\right)
\end{align*}
by which we have
\begin{equation}\label{e:feature-2}
L_i^{\heavy} \geq \frac{\feature_i - 1}{ \frac{m}{C_i} - \frac{1}{L_i}}
\end{equation}
By adding both sides of (\ref{e:feature-1}) and (\ref{e:feature-2}) we get
\begin{align}
& L_i = L_i^{\light} + L_i^{\heavy} \geq \frac{\feature_i - 1}{ \frac{1}{L_i} - \frac{1}{C_i}} + \frac{\feature_i - 1}{ \frac{m}{C_i} - \frac{1}{L_i}} \\
\Rightarrow ~~& \feature_i  \leq 1 + \frac{1}{\frac{1}{1 - \frac{L_i}{C_i}} + \frac{1}{\frac{m L_i}{C_i} - 1}}
\end{align}
For simplicity, we let $y = \frac{L_i}{C_i}$, and thus we know $y \in (0,1]$. Then the above inequality can be rewritten as
\[
\feature_i  \leq 1 + \frac{(1-y)(my-1)}{(m-1)y}
\]
The maximum of the left hand side of the above inequality in the range of $y \in (0,1]$ occurs at $y = \frac{1}{\sqrt{m}}$ and we have
\[
\feature_i  \leq 2 - \frac{2}{\sqrt{m} + 1}
\]

By adding both sides of (\ref{e:feature-1}) and (\ref{e:feature-2}) we get
\begin{equation}\label{e:feature-2}
L_i = L_i^{\light} + L_i^{\heavy} = \frac{\feature_i - 1}{ \frac{1}{L_i} - \frac{1}{C_i}} + \frac{\feature_i - 1}{ \frac{m}{C_i} - \frac{1}{L_i}}
\end{equation}

%\[
%\feature_i=1 + \frac{C_i^{\heavy}}{C_i} - \frac{L_i^{\heavy}}{L_i} \leq 1 + \frac{m \times L_i^{\heavy}}{C_i} - \frac{L_i^{\heavy}}{L_i} = 1 + L_i^{\heavy}\left( \frac{m}{C_i} - \frac{1}{L_i}\right)
%\]


\begin{equation*}
% \nonumber % Remove numbering (before each equation)
\feature_i=1+\frac{L_i^{\light}}{L_i}-\frac{C_i^{\light}}{C_i} \leq 1 + \frac{L_i^{\light}}{L_i} - \frac{L_i^{\light}}{C_i}
= 1 + L_i^{\light}\left( \frac{1}{L_i} - \frac{1}{C_i}\right)
\end{equation*}
\[
\feature_i=1 + \frac{C_i^{\heavy}}{C_i} - \frac{L_i^{\heavy}}{L_i} \leq 1 + \frac{m \times L_i^{\heavy}}{C_i} - \frac{L_i^{\heavy}}{L_i} = 1 + L_i^{\heavy}\left( \frac{m}{C_i} - \frac{1}{L_i}\right)
\]
therefore,
\[
\frac{\feature_i - 1}{\frac{1}{L_i} - \frac{1}{C_i}} + \frac{\feature_i - 1}{\frac{m}{C_i} - \frac{1}{L_i}} \leq L_i
\]
\[
(\feature_i - 1)(\frac{1}{\frac{1}{L_i} - \frac{1}{C_i}} + \frac{1}{\frac{m}{C_i} - \frac{1}{L_i}}) \leq L_i
\]
\[
\feature_i  \leq 1 + \frac{L_i}{\frac{1}{\frac{1}{L_i} - \frac{1}{C_i}} + \frac{1}{\frac{m}{C_i} - \frac{1}{L_i}}}
\]
\[
\feature_i  \leq 1 + \frac{L_i}{\frac{L_i}{1 - \frac{L_i}{C_i}} + \frac{L_i}{\frac{m L_i}{C_i} - 1}}
\]
\[
\feature_i  \leq 1 + \frac{1}{\frac{1}{1 - \frac{L_i}{C_i}} + \frac{1}{\frac{m L_i}{C_i} - 1}}
\]
let $y = \frac{L_i}{C_i}$ which is $\leq 1$
\[
\feature_i  \leq 1 + \frac{1}{\frac{1}{1 - y} + \frac{1}{my - 1}}
\]
\[
\feature_i  \leq 1 + \frac{(1-y)(my-1)}{(m-1)y}
\]

\end{proof}
}
%slightly revising our decomposition strategy.
%Recall that the timing diagram of a task is constructed assuming it executing on infinitely many processors.
%Therefore, the maximal parallelism of each segment could be larger than the number of processors $m$.
%In this case, the extra parallelism beyond $m$ actually does not make any sense since at most $m$ different vertices
%can execute at the same time instant. So we may introduce some artificial edges to the original task graph
%to limit its maximal parallelism degree to at most $m$. More specifically,
%we can check the maximal number of vertices that cover a segment. If this number is larger than $m$, then
%we can arbitrarily choose a pair of them and add an edge between them, and in this way the maximal parallelism
%of this segment is reduced by $1$. We can then repeat this procedure, until the maximal parallelism of
%all segments are bounded by $m$.
%
%In general, we may limit the maximal parallelism of a task to







% \begin{figure}[!t]
%\centering
%\includegraphics[width=2in]{fig5.jpg}
%% where an .eps filename suffix will be assumed under latex,
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%% via \DeclareGraphicsExtensions.
%\caption{An worst case example of DAG $\tau_i$.}
%\label{fig5}
%\end{figure}

%\todo{the worst-case example has been shown before??}
%
%  Therefore, for any given task set of DAGs, we can provide a sufficient schedulability test which depend on three parameters:$\feature_{\maximum}$, $\dendemax_{\summation}$ and $\compress_{\maximum}$. The efficiency of scheduling is largely depending on the structure characteristic value of the DAGs in the task set. We believe that $\Omega_i$ is a good description of the structural feature of the DAGs such that decomposed each DAG $\tau_i$ with the guideline of $\feature_i$ will get us a tighter schedulability test condition.
%
%   \xuadd{We can be find that the value of $\feature_i$ is largely depended on the degree of the uniformity of the task load}, and by making our decomposition process under the guideline of $\feature_i$ would dramatically introduce a load balance during the decomposed subtasks such that the resource requirements could be smaller bounded.
%Since for each light segment $s_i^l$ we have $\frac{c(s^l)}{e(s^l)}<\frac{C_i}{L_i}$ such that

%\begin{equation*}
% \frac{\sum_{l=1}^{n}c(s^l)}{\sum_{l=1}^{n}e(s^l)}=\frac{C_i^{\light}}{L_i^{\light}}<\frac{C_i}{L_i}
% \end{equation*}

%%Hence we have
%\todo{!!!!!!!!!!!!one hour to do this!!}
%the maximum of $\frac{(1-y)(my-1)}{(m-1)y}$ with $y \in (0,1]$ is

%
%
%From the definition of $C_i^{\heavy}$ and $L_i^{\light}$, we have $\frac{C_i^{\heavy}}{C_i}\leq1$ and $\frac{L_i^{\light}}{L_i}\leq1$,due to $\frac{C_i^{\heavy}}{C_i}$ and $\frac{L_i^{\light}}{D_i}$ could not be equal to 1 at the same time , hence $\feature_i<2$.Note that $\feature_i=1$ when there are no light segments  where $ L_i^{\light}=C_i^{\light}=0$. Such that the value of $\feature_i$ is in the range [1, 2). For some terrible DAG, like the DAG $\tau_i$ shown in Fig.6 where $\nu$ and $n$ are very large numbers and $\varepsilon$ is very tiny and the deadline is $\nu+\varepsilon$. DAG $\tau_i$ in Fig.6 has a large $L_i^{\light}$ and a large $C_i^{\heavy}$ which will cause $\feature_i$ to be close to 2. In practical, such extreme case is not much possible exist, for most other DAGs, $\feature_i$ could be much smaller. It can be observed that $\feature_i$ is smaller when the DAG’s load is more uniform. So in order to make the scheduling more efficient, the programmer should try to make the load of the parallel application more uniform.
%
%
%
%%!!!!!!!!!!!!!!!!!!!!!
Finally, with a similar proof to which for Theorem \ref{t:capacity}, we can generalize Theorem \ref{theo4}
to $s$-speed processors:
\begin{corollary}
The resulting sporadic task set by decomposing the parallel task set $\tau$ is schedulable on a $s$-speed processor platform
\begin{equation}
s\geq{\frac{\feature_{\maximum}\util_{\summation}}{m}+\feature_{\maximum}\compress_{\maximum}(1-\frac{1}{m})}
\label{eq31}
\end{equation}
\end{corollary}

==> segmentation-second.tex <==
\subsection{Second Look into Segmentation}\label{ss:segmentation-second}

We use an \emph{ordered} list $\segset$ to store the vertices that have not been assigned to any segment,
and use $\segset^x$ to store the vertices that have already been assigned to segment $s^x$.
Initially, $\segset$ contains all the vertices of $\tau_i$, and each $\segset^x$ is empty.
The elements in $\segset$ are ordered in the increasing order of their latest finish times
(ties are broken arbitrarily).
The elements in $\segset$ will be moved to each $\segset^x$ at the end of the segmentation procedure.
The pseudo-code of our segmentation algorithm is shown in Algorithm \ref{al:segmentation},
which consists of three phases:
\begin{description}
\item[\textbf{\hspace{-4mm}Phase 1:}] \textbf{Assign each vertex that only covers a single segment.} This phase is from line \ref{ln:phase-one-begin} to  \ref{ln:phase-one-end} in Algorithm \ref{al:segmentation}. Each vertex that covers only one segment $s^x$ is simply moved from $\segset$ to $\segset^x$.


\item[\textbf{\hspace{-4mm}Phase 2:}] \textbf{Assign the the remaining vertices to light segments as much as possible, without turning any
light segment into heavy.}
This phase is from line  \ref{ln:phase-two-begin} to \ref{ln:phase-two-end}.
In this phase, we do assignment to each light segments one by one, in the time order (line \ref{ln:phase-two-begin}).
For each light segment $s^x$, we assign vertices that cover $s^x$, according to their order in $\segset$.
A vertex $u$ can be entirely assigned to segment $s^x$ if $s^x$ still remains light after added in the execution time
of $u$  (line \ref{ln:condition}). In this case, we move $u$ from $\segset$ to $\segset^x$ (\ref{ln:entire}),
and go into the next iteration, to assign the next vertex in $\segset$ that covers $s^x$.
Otherwise, we split $u$ into two parts $u'$ and $u''$ such that
after adding $u'$ to $s^x$, $c(s^x)$ exactly reaches $C_i/L_i$, which is the threshold for being transformed
from a light segment to a heavy one.
In this case, the vertex assignment to the current segment is over,
and we put the remaining part $u''$ back to $\segset$ for future assignment to later segments.

\item[\textbf{\hspace{-4mm}Phase 3:}] \textbf{Assign the remaining vertices, if any, to
the heavy segments arbitrarily.}
This phase is from line \ref{ln:phase-three-begin} to \ref{ln:phase-three-end}. After Phase 2, the remaining
elements in $\segset$ can only be assigned to heavy segments (including those segments that just reach
the threshold in Phase 2). Since $\feature_i$ only depends on the total execution time in all heavy segments (i.e., $C_i^\heavy$),
we can assign a remaining element in $\segset$ to its covered segments arbitrarily.
The only constraint is that the part of a vertex assigned to a segment $s^x$ is at most $e(s^x)$.
\end{description}


%%%we first update the $\start(u)$ of each element $u$ in $\segset$
%%%to be the start time of segment $s_i^x$, then reorder all the elements in the increasing order
%%%of their $\finish(u)$.
%%
%%Then we assign vertices that cover $s_i^x$ according to their order in $\segset$.
%
%\todo{not clear, need rewriting ...}


\begin{algorithm}
\caption{The segmentation algorithm.}
\begin{algorithmic}[1]
\FOR {each element $v$ in $\segset$} \label{ln:phase-one-begin}
    \IF{$v$ only covers a single segment $s^x$}
			 \STATE $\segset^x  \gets \segset^x \cup \{ v \}$, ~~$\segset  \gets \segset \setminus \{ v \}$
    \ENDIF
\ENDFOR         \label{ln:phase-one-end}

 \FOR {each light segment $s^x$, $x \in [1, \cdots, X]$} \label{ln:phase-two-begin}
        \FOR{each $u \in \segset$ that covers $s^x$ , in their order in $\segset$ } \label{ln:element-order}
            \IF{$\left(   \frac{ c(u) + \sum_{v\in \segset^x} c(v)}{e(v)} < \frac{C_i}{L_i} \right)$} \label{ln:condition}
    			 \STATE $\segset^x  \gets \segset^x \cup \{ v \}$; ~$\segset  \gets \segset \setminus \{ v \}$;  \label{ln:entire}
            \ELSE
                 \STATE split $u$ into $u'$ and $u''$, such that
                 \[ \frac{ c(u) + \sum_{v\in \segset^x} c(v)}{e(v)} = \frac{C_i}{L_i};\]
%                 \STATE $(u', u'') = Split(u)$;
                 \STATE $\finish(u'') \gets \finish(u)$;
                 \STATE $\segset^x  \gets \segset^x \cup \{ u' \}$;
                 \STATE $\segset  \gets (\segset \setminus \{ u \}) \cup \{ u'' \}$ // $u''$ be the head of $\segset$
                 \STATE \textbf{break}; \label{ln:break}
            \ENDIF
        \ENDFOR
\ENDFOR  \label{ln:phase-two-end}

\IF{$\segset$ is not empty} \label{ln:phase-three-begin}
    \STATE{Arbitrarily assign the remaining elements in $\segset$ to their
    related segments;
    }
\ENDIF  \label{ln:phase-three-end}
%    \FOR {each element $v$ in $\segset$}
%        \FOR {each segment $e(s_i^x)$ covered by $v$}
%            \IF{$c(v) \leq e(s_i^x)$}
%                \STATE $\segset^x  \gets \segset^x \cup \{ v \}$, ~~$\segset  \gets \segset \setminus \{ v \}$
%            \ELSE
%                \STATE split $v$ into $v'$ and $v''$, such that $c(v') = e(s_i^x)$
%            \STATE $\segset^x  \gets \segset^x \cup \{ v' \}$, ~~ $\segset  \gets (\segset \setminus \{ v \}) \cup \{ v'' \}$
%            \ENDIF
%        \ENDFOR
%    \ENDFOR

\end{algorithmic}\label{al:segmentation}
\end{algorithm}

We use our running example in Figure \ref{fig1} and \ref{fig2} to illustrate Algorithm \ref{al:segmentation}. In phase 1, $v_1$ is assigned to $s^1$,
$v_3$ to $s^2$, $v_5$ to $s^3$, $v_6$ and $v_7$ to $s^4$ and $v_8$ to $s^5$.
In phase 2, we visit each segment in time order.
\begin{itemize}
\item $s^1$: nothing can be assigned.
\item $s^2$: there are two vertices $v_2$ and $v_4$ covering $s^2$.
$v_4$ is before $v_2$ in $\segset$ since $\finish(v_4) < \finish(v_2)$.
$v_4$ is split into two parts $v_4'$ and $v_4''$
so that $(c(v_3) + c(v_4'))/e(s^2) = C_i/L_i = 2$, which implies $c(v_4') = c(v_4'') = 4$.
Then we assign $v_4'$ to $s^2$ and put $v_4''$ back to $\segset$ for future use.
\item $s^3$: Both $v_2$ and $v_4''$ cover $s^2$, and $\finish(v_4'')$ which inherits from
$\finish(v_4)$ is earlier than $\finish(v_2)$. After assigning entire $v_4''$ to it, $s^3$ is still
light, so we will continue to assign $v_2$ to $s^3$. We split $v_2$ into two parts $v_2'$ and $v_2''$,
with $c(v_2')=1$ and $c(v_2'')=2$, such that $(c(v_5) + c(v_4'') + c(v_2'))/e(s^3) = C_i/L_i = 2$, and
put $v_2''$ back to $\segset$.
\item $s^4$: This segment, although light, already meets the threshold, i.e., $(c(v_6) + c(v_7))/e(s^4) = C_i/L_i = 2$,
therefore no assignment in this phase.
\item $s^5$: nothing can be assigned.
\end{itemize}
After Phase 2, $v_2''$ is the only remaining element in $\segset$, and we can arbitrarily assign it to any segment covered by it.
We choose to assign it to $s^4$, and the final result of the segmentation is shown in Figure \ref{fig2-seg}.


% \begin{figure}[!t]
%\centering
%\includegraphics[width=2in]{fig_segmentation.jpg}
%% where an .eps filename suffix will be assumed under latex,
%% and a .pdf suffix will be assumed for pdflatex; or what has been declared
%% via \DeclareGraphicsExtensions.
%\caption{\xuadd{The segmentation of DAG $\tau_i$.}}
%\label{fig.segmentation}
%\end{figure}

%\xuadd{Fig.\ref{fig.segmentation} shows the segmentation process of task $\tau_i$ in Fig.\ref{fig1}.}

\begin{theorem}\label{th:optimal-segmentation}
The segmentation algorithm in Algorithm \ref{al:segmentation} is optimal in the sense of resulting in the minimal $\feature_i$.
\end{theorem}
The proof of the Theorem \ref{th:optimal-segmentation} is provided in the Appendix.
There are two keys for Algorithm \ref{al:segmentation} to be optimal. First, we always try to assign
vertices to light segments to make their $\frac{c(s^x)}{e(s^x)}$ to just reach the threshold $\frac{C_i}{L_i}$.
Therefore, these segments will not turn into heavy segments, and thus the assigned workload will not be
counted into $\feature_i$. Second, in Phase 2, the workload of different vertices are assigned to light segments in an EDF-like manner,
which ensures the optimality of allocating their workload to let as many light segments meet the threshold as possible.

%\todo{proof idea: after phase 2, the total amount of remaining unassigned execution should be minimal. this can
%be proved by contradiction, assuming there is another strategy that assigns more than ours in phase 2.}


==> segmentation.tex <==
%\subsection{Segmentation}

The timing diagram of a task $\tau_i$ (of length $T_i$)
is divided into several segments by the earliest ready time $\start(v)$ of
each vertex $v$.
In general, the lifetime window $[\start(v) , \finish(v) ]$ of a vertex $v$
may cover several segments.
In this case, a vertex can be assigned to one or more of these segments
(a vertex may be split into several parts and each part is assigned to one
of these segments).
Later in Section \ref{ss:segmentation-second} we will introduce how to
assign the vertex to these segments, and will see how this will affect the
schedulability of the task set. For this moment, we just assume that
each vertex $v$ has been assigned to one or more of these segments covered by its lifetime window $[\start(v) , \finish(v) ]$.


 Assume a task is divided into $X$ segments, and we use
$s^1, \cdots, s^X$ to denote these segments, and we use
$e(s^x)$ to denote the length of segment $s^x$, and
$c(s^x)$ to denote the total amount of workload of every vertex (or a part of a vertex) assigned to segment $s^x$,
and we know
\begin{equation}
L_i = \sum_{x = 1}^X e(s^x), ~C_i = \sum_{x = 1}^X c(s^x)
\end{equation}


%
%Each segment consists of several threads while each thread corresponds to a part of a vertex lies in the segment
%(or a vertex that completely fall in this segment). Thus, $e_i^x$ is also the length of the longest thread
%in segment $e_i^x$. Moreover, we
%use $c_i^x$ to denote the total amount of all threads  in segment $s_i^x$.
%
%In this case, we will distribute
%the execution time of this vertex to these segments, with each part
%propositional to the length of each
%involved segment.





Finally, we classify all the segments into two types:
\begin{define}\label{d:light-heavy}
$s^x$ is a \emph{light segment} if
\[
\frac{c(s^x)}{e(s^x)} \leq \frac{C_i}{L_i}
\]
and is a \emph{heavy segment} otherwise.
 We use $\light_i$ and $\heavy_i$ to denote the set of light and heavy segments of task $\tau_i$, respectively.
\end{define}



Figure \ref{fig2-seg} shows the segmentation of the task in Figure \ref{fig1},
where the timing diagram is divided into $5$ segments, and $v_2$ (the one with $c(v_2) = 3$)
covers segments $s^2, s^3, s^4$ and $v_4$ covers $s^2, s^3$.
Suppose we split the workload of $v_2$ into two parts $1$ and $2$ and assign them to $s^3$ and $s^4$,
and split $v_4$ into two equal parts and assign them to $s^2$ and $s^3$
(here we only use this example to illustrate the related concepts,
and the concrete segmentation strategy will be presented later in Section \ref{ss:segmentation-second}).
In this case, we know the classification of each segment as follows ($C_i/L_i = 30/15 = 2$):
\begin{align*}
s^1: ~& c(s_1)/e(s_1) = 1 < 2 \Rightarrow \textrm{light} \\
s^2: ~& c(s_2)/e(s_2) = 8/4 = 2 \Rightarrow \textrm{light} \\
s^3: ~& c(s_3)/e(s_3) = 10/5 = 2 \Rightarrow \textrm{light} \\
s^4: ~& c(s_4)/e(s_4) = 10/4 > 2 \Rightarrow \textrm{heavy} \\
s^5: ~& c(s_5)/e(s_5) = 1/1 < 2 \Rightarrow \textrm{light}
\end{align*}









==> segmentation_proof.tex <==
\section*{Appendix: Proof of Theorem \ref{th:optimal-segmentation}}

\begin{proof}
After the segmentation the total amount of workload assigned to a heavy segment $s^h$ is $c(s^h)$.
We define
\[
c_{out}(s^h) =  c(s^h) - C_i/L_i \times e(s^h)
\]
Recall that a segment is heavy if  $c(s^h)/e(s^h) > C_i/L_i$,
so $c_{out}(s^h)$ is the part of \enquote{overflowed} workload in $s^h$ that make 
$c(s^h)/e(s^h)$ above $C_i/L_i$.
Then we define 
\[
C_{out} =  \sum_{s^h \in \heavy} c_{out}(s^h)
\]
The proof of the theorem goes into two steps. 
\begin{enumerate}
\item First we prove that $\feature_i$ is minimized iff $C_{out}$ is minimized.
\item Second we prove that our segmentation algorithm leads to the minimal $C_{out}$.
\end{enumerate}
We start with the first step, by the definition of $\feature_i$
\begin{align*}
\feature_i &= \frac{C_i^{\heavy}}{C_i}+\frac{L_i^{\light}}{L_i} = \frac{(L_i - L_i^{\light} ) \frac{C_i}{L_i} + C_{out}}{C_i} +  \frac{L_i^{\light}}{L_i} = 1 + \frac{C_{out}}{C_i}
\end{align*}
Therefore, the first step is proved. The remaining of the proof dedicates to the second step.

The proof of the second step uses the \enquote{time slice swapping} technique, which was used
to prove the optimality of EDF scheduling algorithm on single-processors \cite{dertouzos74edf}.
We first compare our segmentation algorithm and EDF scheduling algorithm, to show their similarity and
difference. Then we will show how to adopt the \enquote{time slice swapping} technique for proving the
optimality of EDF scheduling to our problem.

In our segmentation problem, the time line is divided into segments by the earliest ready time and latest finish time
of each vertex. At the beginning of our segmentation algorithm in Algorithm \ref{al:segmentation},
each segment is empty. For each segment $s$, $e(s) \times \frac{C_i}{L_i}$ it can receive
in the time interval of length $e(s)$, without being turned into a heavy segment.
Therefore, we can normalize $c(v)$ of each vertex $v$ by $c'(v) = c(v) \times \frac{L_i}{C_i} $,
such that the assignment of each vertex can be seen as schedule a job
on a unit-speed single-processor, whose worst-case execution time is $c'(v)$, release time is
the earliest ready time $\start(v)$ of $v$ and deadline is the latest finish time $\finish(v)$ of $v$.
The execution of this job for $t$ time units in the range of a segment
corresponds to assigning $t \times \frac{C_i}{L_i}$
workload of $v$ to this segment. The
The job can only execute between its release time and deadline, since a vertex $v$ can only be assigned
to segments between its earliest ready time $\start(v)$ and latest finish time $\finish(v)$.
In the first two phases of Algorithm \ref{al:segmentation}, the assignment to each segment
is prioritized among vertices in that way that it always selects the vertex $v$ with the earliest $\finish(v)$
to be assigned (or one of them in case there are several). Therefore, the corresponding jobs are scheduled by EDF.

Although similar, our segmentation problem is not exactly the same as the real-time scheduling problem
of the corresponding jobs. The difference is that, in real-time scheduling the target is to make all
the jobs to meet their deadlines, while in our segmentation problem some vertex may not be completely
assigned to segments by the point when none of the segments can be further assigned without being turned
into heavy. Then the remaining workload of these vertices will be assigned to heavy segments in the
third phase, which will all contribute to $C_{out}$. Since we want to minimize $C_{out}$ and thus $\feature_i$, we should
make the total amount of leftover workload
of all the vertices as small as possible before starting assign to heavy segments
If we interpret this in the form of scheduling the vertices' corresponding jobs, our segmentation problem
is equivalently to the following generalized form of real-time scheduling problem:
~~\\

\vspace{-3mm}
\textbf{\underline{General Real-Time Scheduling Problem}: }\emph{Given a set of real-time jobs with known release times and deadlines. Each job can only execute between its release time and deadline, and in general it may have a certain amount of unfinished workload
by its deadline. Then how to schedule these jobs on a single-processor so that the total amount of unfinished workload of all jobs
does not exceed a threshold $\triangle$?}
\vspace{-3mm}

~~\\
Note that the standard real-time scheduling problem is a special case of the above defined problem, with $\triangle = 0$.
In the following we will show that EDF scheduling is still optimal with this general real-time scheduling problem.
This can be proved using the \enquote{time slice swapping} proof technique. We define say a schedule is valid
if each the job executes between its release time and deadline, and the total amount of unfinished workload of all jobs is at most $\triangle$. Then the following procedure is essentially the same
as that for EDF optimality in the standard real-time scheduling problem \cite{dertouzos74edf}.
The only difference is that for in the standard real-time scheduling problem
the swapping of execution of a job to an earlier point won't cause it to miss deadline,
while in our general real-time scheduling problem such a swapping won't increase
the total amount of


We will prove that any valid schedule for this job set can
be transformed into a valid EDF schedule. This will be shown
by induction on $t$: the transformation is possible for any time interval $[0, t)$.
This is trivially true for $t = 0$. Now assume
it is true for time interval $[0, t)$ that a job with deadline $d_j$
is executed in the time interval $[t, t + 1)$, and that the earliest deadline
among all jobs pending at $t_1$ is $d_i < d_j$. Let $t'$ be the first time
at which the job with deadline $d_i$ is executed after $t$. We know that
$t < t'$ and $t' < d_i < d_j$.
Therefore, by swapping the executions in $[t, t+1)$ and
$['t, t'+1)$ no deadline violation occurs in $[t, t+1)$,
and thus no extra unfinished workload is introduced in $[t, t+1)$. By the inductive hypothesis
we know the total amount of unfinished workload is no more than $\triangle$
by time $t$, so in summary the total amount of unfinished workload is no more than
than $\triangle$ by time $t+1$.

By now we have proved EDF is still optimal for General Real-Time Scheduling Problem
\end{proof}
%
%Let us draw a threshold window whose length is $L_i$ and width is $C_i/L_i$. The window is divided into two kinds of segments by the release time and relative deadline of all vertex: the segments is fully loaded(heavy segments) and other segments with slack in it(light segments). Suppose that for an arbitrary valid segmentation(we say a segmentation is valid if all the vertexes could only be put in the segment that the release time of the vertex is no later than the beginning of the segment. The deadline of the vertex is no less than the end of the segment is automatic guaranteed because the window is split according to the release time and relative dead line of all vertexes ), there are some "execution time" falls in the window and some parts of threads out the window which could not be put in the window. Let $C_{out}$ denoted the total execution time out of the window, then we can calculate $\feature_i$ to be $1+\frac{C_{out}}{C_i}$.
%
%
%\begin{proof}
%From the definition of $\feature_i$ we have:
%\begin{equation*}
%\feature_i=\frac{C_i^{\heavy}}{C_i}+\frac{L_i^{\light}}{L_i}
%\end{equation*}
%
%For all segments falls in the window, they are either light segments of heavy segments with total density exactly $C_i/L_i$. Suppose that all heavy segments have total length of $\alpha$, and all light segments with total length of $\beta$ where $\alpha+\beta=L_i$.Hence the $\feature_i$ is :
%\begin{equation}
%\frac{\frac{\alpha{C_i}}{L_i}+C_{out}}{C_i}+\frac{\beta}{L_i}=1+\frac{C_{out}}{C_i}
%\label{equ.cout}
%\end{equation}
%
%\end{proof}
%
%Then for all segmentations,from equation \ref{equ.cout} we have the $\feature_i$ is minimum when $C_{out}$ is minimum. Such that the optimal segmentation is when we make the vertex falls in the window as much as possible.
%
%
%\begin{theorem}
%The Algorithm \ref{algrithm x} is an optimal segmentation if there exists any valid segmentation which makes $C_{out}$ to be minimum, then segmentation of Algorithm.\ref{algorithm x} can makes $C_{out}$ to be minimum.
%\end{theorem}
%
%
%\begin{proof}
%It is obvious that the Phase 1 in Algorithm \ref{algrithm x} is identical for any segmentation. Suppose that after Phase 1 there are $s$ light segments with slack. Then the problem is transformed into that to put the execution time of the remaining vertexes in these slacks as much as possible. In Phase 2 of Algorithm \ref{algrithm x}, we always fill the slack of each segment with the pending vertex by the earliest deadline order. Now we need to prove that if there is another valid segmentation can put $\alpha$(a arbitrary value which is no more than the total slack time) time in the window then by Algorithm \ref{algrithm x} can also put $\alpha$ time in it.
%
%The proof is similar with the optimal proof of EDF on single processor.
%
%Let $t_0$ denoted the release time of the fist light segment after Phase 1.The theorem is obvious true for $t_0$. For the first light segment, the total execution time of the pending vertexes is the same for both segmentation, such that if the other segmentation put $T_1$ time in the segment, then by Algorithm \ref{algrithm x} could also put $T_1$ time in the segment. Assume now that the total execution time that been put by Algorithm \ref{algrithm x} and another segmentation in the threshold window is the same before the $j-th$ light segment. Let $C_{before}$ denotes the total execution time of the vertexes with deadline no later than the end of $j-1-th$ light segments and $C_{later}$ denotes the total execution time of the vertexes with deadline no earlier than the end of $j-th$ light segment.Then by Algorithm \ref{algrithm x}, after the segmentation of all the $j-1-th$ light segments, the remaining execution time of $C_{before}$ is denoted by $C_1$ while for other segmentation is $C_1^{'}$ and the remaining time of $C_{later}$ is denoted by $C_2$ while for the other segmentation is $C_2^{'}$. Because of that by Algorithm \ref{algrithm x} is always put the vertexes with earliest deadline in each light segment such that we have $C_2\geq{C_2^{'}}$. Hence that,the total pending execution time for the $j-th$ light segment by Algorithm \ref{algrithm x} is no less than the other one, then if the other segmentation can put $T_2$ time in the segment,then by Algorithm \ref{algrithm x} could also put $T_2$ time in the segment.
%Such that for all the light segments if a segmentation could put $\alpha$ time in the window then by Algorithm \ref{algrithm x} could also put $\alpha$ time in the window. Hence follow the theorem.
%
%
%

%\end{proof}

==> semi_federated.tex <==
\section{semi-federated scheduling}\label{s:semi_federated}












